Q-SLAM: Quadric Representations for Monocular SLAM

In this paper, we reimagine volumetric representations through the lens of quadrics. We posit that rigid scene components can be effectively decomposed into quadric surfaces. Leveraging this assumption, we reshape the volumetric representations with million of cubes by several quadric planes, which results in more accurate and efficient modeling of 3D scenes in SLAM contexts. First, we use the quadric assumption to rectify noisy depth estimations from RGB inputs. This step significantly improves depth estimation accuracy, and allows us to efficiently sample ray points around quadric planes instead of the entire volume space in previous NeRF-SLAM systems. Second, we introduce a novel quadric-decomposed transformer to aggregate information across quadrics. The quadric semantics are not only explicitly used for depth correction and scene decomposition, but also serve as an implicit supervision signal for the mapping network. Through rigorous experimental evaluation, our method exhibits superior performance over other approaches relying on estimated depth, and achieves comparable accuracy to methods utilizing ground truth depth on both synthetic and real-world datasets.

==> tables/ablation.tex <==
\begin{table}[htpb]
	\centering
	% \footnotesize
	\begin{center}
 	\caption{Ablation study on Replica dataset.}	
  % \vspace{-5pt}
	\label{table:ablation}
		% \resizebox{1.0\textwidth}{!}
		{
			\begin{tabular}{l|l||cc|c}
				\toprule
				%\multicolumn{2}{c|}{\text { 2D Metrics }} & \multicolumn{4}{c}{\text { 3D Metrics }}
				&   & Depth L1 [cm] $\downarrow$ & PSNR [dB] $\uparrow$ & ATE RMSE [cm] $\downarrow$\\
				%\midrule
				\noalign{\smallskip}
				\hline\hline
				%\cline{1-26}
				\noalign{\smallskip}
				\multirow{2}{*}{ (a) }  
				& Ours (w/o quadric depth correction)  
				& 5.63 & 32.55
				& 0.48 
				\\
				&Ours (full, with quadric depth correction)     
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
				\noalign{\smallskip}
                \cline{1-5}\noalign{\smallskip}
				\multirow{3}{*}{ (b) }     
				& Ours (w/o quadric ray transformer)  
				& 5.02 & 33.13
				& 0.47 
				\\
    				& Ours (w only intra-ray transformer)  
				& 4.36 & 34.78
				& 0.44
				\\
				&Ours (full, with quadric ray transformer)     
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
				\noalign{\smallskip}
                \cline{1-5}\noalign{\smallskip}
				\multirow{2}{*}{ (c) }     
				& Ours (w/o joint optimization)  
				& 4.42 & 34.21
				& 0.41 
				\\
				& Ours (full, with joint optimization)   
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
                \cline{1-5}\noalign{\smallskip}
				\multirow{2}{*}{ (d) }     
				& Ours (w/o semantic supervision)  
				& 5.87 & 31.18
				& 0.51 
				\\
				& Ours (full, with semantic supervision)   
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
				\bottomrule
			\end{tabular}
		}
	\end{center}
 % \vspace{-20pt}
\end{table}


==> tables/ablation_new.tex <==
\begin{table}[htpb]
	\centering
	% \footnotesize
	\begin{center}
 	\caption{The ablation study of mapping and tracking on Replica dataset \texttt{office0}.}	
  % \vspace{-5pt}
	\label{table:ablation}
		% \resizebox{1.0\textwidth}{!}
		{
			\begin{tabular}{l|l||cc|c}
				\toprule
				%\multicolumn{2}{c|}{\text { 2D Metrics }} & \multicolumn{4}{c}{\text { 3D Metrics }}
				&   & Depth L1 [cm] $\downarrow$ & PSNR [dB] $\uparrow$ & ATE RMSE [cm] $\downarrow$\\
				%\midrule
				\noalign{\smallskip}
				\hline\hline
				%\cline{1-26}
				\noalign{\smallskip}
				\multirow{2}{*}{ (a) }  
				& Ours (w/o quadric depth correction)  
				& 5.63 & 32.55
				& 0.48 
				\\
				&Ours (full, with quadric depth correction)     
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
				\noalign{\smallskip}
                \cline{1-5}\noalign{\smallskip}
				\multirow{3}{*}{ (b) }     
				& Ours (w/o quadric ray transformer)  
				& 5.02 & 33.13
				& 0.47 
				\\
    				& Ours (w only intra-ray transformer)  
				& 4.36 & 34.78
				& 0.44
				\\
				&Ours (full, with quadric ray transformer)     
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
				\noalign{\smallskip}
                \cline{1-5}\noalign{\smallskip}
				\multirow{2}{*}{ (c) }     
				& Ours (w/o joint optimization)  
				& 4.42 & 34.21
				& 0.41 
				\\
				& Ours (full, with joint optimization)   
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
                \cline{1-5}\noalign{\smallskip}
				\multirow{2}{*}{ (d) }     
				& Ours (w/o semantic supervision)  
				& 5.87 & 31.18
				& 0.51 
				\\
				& Ours (full, with semantic supervision)   
				& \textbf{3.29} & \textbf{36.31}
				& \textbf{0.39}
				\\
				\bottomrule
			\end{tabular}
		}
	\end{center}
 % \vspace{-20pt}
\end{table}


==> tables/replica_new.tex <==
\setlength{\tabcolsep}{0.7mm}
% \renewcommand{\arraystretch}{1.08}
\begin{table}[tpb]
\centering
\caption{Photometric (PSNR [dB], SSIM, LPIPS) and Geomertric (Depth L1 [cm]) results on Replica dataset \cite{straub2019replica}. Higher PSNR values mean better color rendering performance and lower Depth L1 values denote better depth reconstruction.}
\label{tab:Replica_details}
\resizebox{1.\textwidth}{!}{
\begin{tabular}{clccccccccc}
\toprule
Method  & Metric & \texttt{Room0} & \texttt{Room1} & \texttt{Room2} & \texttt{Office0} & \texttt{Office1} & \texttt{Office2} & \texttt{Office3} & \texttt{Office4} & Avg.  \\
\midrule
\multirow{4}{*}{\makecell[c]{$\textbf{Nice-SLAM}$\cite{zhu2022nice} \\(GT depth)}} 
& PSNR $\uparrow$ & 22.12  & 22.47  & 24.52  & 29.07    & 30.34    & 19.66    & 22.23    & 24.94    & 24.42 \\
& SSIM $\uparrow$     & 0.63  & 0.75  & 0.81  & 0.87    & 0.88    & 0.79    & 0.85    & 0.89    & 0.83 \\
& LPIPS $\downarrow$    & 0.33  & 0.27  & 0.20  & 0.22    & 0.18   & 0.23    & 0.20    & 0.19    & 0.23 \\
& Depth L1 $\downarrow$ & 3.53 & 3.60 & 3.03 & 5.56 & 3.35 & 4.71 & 3.84 & 3.35 & 3.87 \\
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{Vox-Fusion} \cite{yang2022vox} \\(GT depth)}} 
 & PSNR $\uparrow$ & 22.39  & 22.36  & 23.92  & 27.79    & 29.83    & 20.33    & 23.47    & 25.21    & 24.41 \\
& SSIM $\uparrow$     & 0.68  & 0.75  & 0.79  & 0.85    & 0.87    & 0.79    & 0.80    & 0.84    & 0.80 \\
& LPIPS  $\downarrow$   & 0.30  & 0.26  & 0.23  & 0.24    & 0.18    & 0.24    & 0.21    & 0.19    & 0.23 \\
& Depth L1 $\downarrow$ & 2.51 & 1.69 & 3.37 & 2.55 & 2.08 & 3.03 & 2.89 & 2.86 & 2.67 \\
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{SplaTAM} \cite{keetha2023splatam} \\(GT depth)}} 
 & PSNR $\uparrow$ & 32.86 & 33.89 & \textbf{35.25} & 38.26 & 39.17 & 31.97 & 29.70 & 31.81 & 34.11\\
 & SSIM $\uparrow$ & \textbf{0.98}  & 0.97  & 0.98  & 0.98  & 0.98  & 0.97  & 0.95  & 0.95 & 0.97 \\
& LPIPS $\downarrow$  &\textbf{0.07}  & \textbf{0.10}  & \textbf{0.08}  & \textbf{0.09}  & \textbf{0.09}  & \textbf{0.10}  & \textbf{0.12 } & 0.15 & 0.10 \\
& Depth L1 $\downarrow$ & \textbf{0.63} &\textbf{0.62} &\textbf{0.98} &\textbf{0.57} &1.66 &7.32 &3.94 &\textbf{0.88}& 2.08\\
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{Ours} \\(GT depth)}} 
 & PSNR $\uparrow$ & \textbf{33.24} & \textbf{34.81} & 34.16 & \textbf{39.32} & \textbf{39.51} & \textbf{34.08} & \textbf{32.65} & \textbf{34.93} & \textbf{35.34} \\
& SSIM $\uparrow$   & \textbf{0.98}  & \textbf{0.99}  & \textbf{0.98}  & \textbf{0.99}  & \textbf{0.99}  & \textbf{0.98}  & \textbf{0.96}  & \textbf{0.98}  & \textbf{0.98}\\
& LPIPS $\downarrow$   & 0.13  & 0.11  & 0.11  & 0.10  & 0.10  & 0.13  & 0.13  & \textbf{0.11}  & 0.12 \\
& Depth L1 $\downarrow$ & 0.82 & 0.77 & 1.35 & 1.74 &\textbf{1.56} &\textbf{4.23} &\textbf{3.23} &1.26& \textbf{1.87}\\
\midrule
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{COLMAP} \cite{schonberger2016structure} \\(Predicted depth)}} 
& PSNR $\uparrow$ & 20.93 & 11.67 & 10.35 & 5.88 & 5.88 & 15.66 & 13.73 & 17.47 & 12.70 \\
& SSIM $\uparrow$ &  0.77 & 0.69 & 0.75 & 0.59 & 0.53 & 0.80& 0.79 & 0.81 & 0.72  \\
& LPIPS $\downarrow$    & 0.29 & 0.44 & 0.33 & 0.44 & 0.33 & 0.30 & 0.29 & 0.27 & 0.34 \\
& Depth L1 $\downarrow$ & 3.87 & 27.29 & 5.41 & 5.21 & 12.69 & 4.28 & 5.29 & 5.45 & 8.69 \\
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{Droid-SLAM} \cite{teed2021droid} \\(Predicted depth)}} 
 & PSNR $\uparrow$ & 18.25 & 18.65& 13.49& 16.13& 10.31 &14.78 &15.53& 15.71 &15.36\\
& SSIM $\uparrow$     & 0.73 & 0.79& 0.78& 0.76& 0.65& 0.80& 0.79& 0.80 &0.76 \\
& LPIPS  $\downarrow$   & 0.35& 0.28& 0.29& 0.29& 0.28 &0.30& 0.30& 0.31& 0.30 \\
& Depth L1 $\downarrow$ & 12.18& 8.35& 3.26& 3.01 &2.39& 5.66& 4.49& 4.65& 5.50 \\
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{Nicer-SLAM}\cite{zhu2023nicer} \\(Predicted depth)}} 
 & PSNR $\uparrow$ & 25.33& 23.92& 26.12& 28.54& 25.86& 21.95 &26.13& 25.47 &25.41\\
 & SSIM $\uparrow$ &0.75& 0.77& 0.83& 0.86& 0.85& 0.82& 0.85& 0.86& 0.82 \\
& LPIPS $\downarrow$  &0.25& 0.21 &0.17& 0.17 &0.17 &\textbf{0.19} &\textbf{0.16}& \textbf{0.17}& 0.19 \\
& Depth L1 $\downarrow$ & 2.53 & 3.93& 3.40& 5.49 &3.45& 4.02& \textbf{3.34}& 3.03 &3.65\\
\midrule
\multirow{4}{*}{\makecell[c]{\textbf{Ours} \\(Predicted depth)}} 
 & PSNR $\uparrow$ & \textbf{29.58} & \textbf{32.74} & \textbf{31.25} & \textbf{36.31} & \textbf{37.22} & \textbf{30.68} & \textbf{30.21} & \textbf{31.96} & \textbf{32.49} \\
& SSIM $\uparrow$   & \textbf{0.83}  & \textbf{0.91}  & \textbf{0.87}  & \textbf{0.94}  & \textbf{0.94}  & \textbf{0.90}  & \textbf{0.88 } & \textbf{0.89}  & \textbf{0.89}\\
& LPIPS $\downarrow$   & \textbf{0.18}  & \textbf{0.16}  & \textbf{0.15}  & \textbf{0.13}  & \textbf{0.15}  & 0.20  & 0.19  & 0.18  & \textbf{0.17} \\
& Depth L1 $\downarrow$ & \textbf{1.32} & \textbf{1.19} & \textbf{2.48} & \textbf{3.29} & \textbf{3.07} & \textbf{3.87} &4.24 &\textbf{2.78}& \textbf{2.76}\\
\bottomrule
\end{tabular}}

% \vspace{-20pt}
\end{table}

==> tables/tum_rgbd.tex <==
% \setlength{\tabcolsep}{1.2mm}
% \renewcommand{\arraystretch}{1.0}
\begin{table}[!htpb]
\centering
        % \resizebox{1.\linewidth}{!}{
\begin{tabular}{lccc}
\toprule & \text { fr1/desk } & \text { fr2/xyz } & \text { fr3/office } \\
\midrule \text { Kintinuous \cite{newcombe2011kinectfusion}} & 0.037 & 0.029 & 0.030 \\
\text { BAD-SLAM \cite{schops2019bad}} & 0.017 & 0.011 & 0.017 \\
\text { ORB-SLAM2 \cite{mur2017orb}} & 0.016 & {\textbf{0.004}} & {\textbf{0.010}} \\
\midrule \text { iMAP \cite{sucar2021imap}  } & 0.049 & 0.020 & 0.058 \\
\text { NICE-SLAM \cite{zhu2022nice} } & 0.027 & 0.018 & 0.030 \\
 \text { GO-SLAM \cite{zhang2023go}} & {0.015} & 0.006 & 0.013 \\
 \midrule
  \text { Ours } & {\textbf{0.014}} & 0.005 & 0.011 \\
\bottomrule
    \end{tabular}
    % }
    \caption{ATE [m] Results on TUM dataset \cite{sturm2012benchmark} with RGB-D inputs from freiburg1, freiburg2 and freiburg3 set. Lower ATE values mean better tracking performance.
}
    \label{tab:tum_rgbd}
\end{table}


==> tables/tum_rgbd_ver.tex <==
% \setlength{\tabcolsep}{1.2mm}
\renewcommand{\arraystretch}{1.0}
\begin{table}[htpb]
    \centering
        % \resizebox{1.\linewidth}{!}{
    \begin{tabular}{cccccccc}
\toprule
Method & \text { Kintinuous \cite{newcombe2011kinectfusion}} & \text { BAD-SLAM \cite{schops2019bad}} & \text { ORB-SLAM2 \cite{mur2017orb}} &   \text { iMAP \cite{sucar2021imap}  } & \text { NICE-SLAM \cite{zhu2022nice} } & \text { GO-SLAM \cite{zhang2023go}} & \text { Ours } \\


\bottomrule
    \end{tabular}
    % }
    \caption{ATE [m] Results on TUM dataset \cite{sturm2012benchmark} with RGB-D inputs from freiburg1, freiburg2 and freiburg3 set. Lower ATE values mean better tracking performance.
}
    \label{tab:tum_rgbd}
\end{table}

